Robust Planning and Control For Polygonal Environments via Linear Programming

We propose a novel approach for navigating in polygonal environments by synthesizing controllers that take as input relative displacement measurements with respect to a set of landmarks. Our algorithm is based on solving a sequence of robust min-max Linear Programming problems on the elements of a cell decomposition of the environment. The optimization problems are formulated using linear Control Lyapunov Function (CLF) and Control Barrier Function (CBF) constraints, to provide stability and safety guarantees, respectively. The inner maximization problem ensures that these constraints are met by all the points in each cell, while the outer minimization problem balances the different constraints in a robust way. We show that the min-max optimization problems can be solved efficiently by transforming it into regular linear programming via the dualization of the inner maximization problem. We test our algorithm to agents with first and second-order integrator dynamics, although our approach is in principle applicable to any system with piecewise linear dynamics. Through our theoretical results and simulations, we show that the resulting controllers: are optimal (with respect to the criterion used in the formulation), are applicable to linear systems of any order, are robust to changes to the start location (since they do not rely on a single nominal path), and to significant deformations of the environment.

==> document.tex <==
%%% Abstract
In this paper we propose a set of controllers, on a cell decomposition of a polygonal environment, based on linear programming. The core of our algorithm consists of a convex min-max formulation that synthesizes an output-feedback controller, based on relative displacement measurements with respect to a set of landmarks. The optimization problem is formulated using piece-wise linear Control Lyapunov Function (CLF) and Control Barrier Function (CBF) constraints, to provide stability and safety guarantees, respectively. The inner maximization problem ensures that these constraints are met by all the points in each cell, while the outer minimization problem balances the constraints to optimize robustness. We convert the min-max optimization problem to a regular linear programming problem, by forming the dual of the inner maximization problem. Although in principle our approach is applicable to any system with piecewise linear dynamics, in this paper as a proof of concept, we apply the approach to first and second order integrators. Simulation results verify the robustness of our proposed controller to significant deformations of the environment. 


---------------------------------------------------------
%%% Introduction

%%%%%%%%%%%%%%%%%%%%%%%% Beginning of the introduction
Motion planning and control of mobile robots is a fundamental problem that has received a growing attention over the last few years \cite{lavalle2006planning}, \cite{latombe2012robot}, \cite{choset2005principles}. Robotic community usually investigates the solution of this problem in two frameworks, namely a path planning framework where the goal is to provide a desired path for the robot from its initial to the goal configuration without colliding obstacles, and a control framework where the objective is to design controller(s) for following the desired path as close as possible. \par
The main assumption in most of the path planning algorithms is that the robot is fully actuated and hence by ignoring the constraints in the dynamical performance of the robot, they just focus on the complexity of the environment. Some of the path planning methods consider a continuous model for the environment and therefore provide a continuous path, such as potential fields \cite{khatib1986real}, \cite{krogh1984generalized} and navigation functions \cite{rimon1992exact}, while the other group solve the planning problem by abstracting the environment to a finite representation and find a discrete path, such as probabilistic roadmaps \cite{kavraki1996probabilistic} and cell decomposition methods \cite{lingelbach2004path}. However, most of these algorithms become computationally inefficient in high-dimensional configuration spaces and hence sampling-based methods were proposed to overcome this problem \cite{lavalle2001randomized}, \cite{karaman2011sampling}.  \par
On the other side, in control algorithms the focus is on kinematic and dynamic constraints on the robot's performance, while assuming simple environments around the robot, such as control algorithms based on input parametrization \cite{morin2000control} or based on differential geometric \cite{lafferriere1993differential} approaches. The main challenge in considering path planning and control algorithms is that the output of the path planning framework may not be possible to perfectly follow in the control framework and requires an interconnection between these two frameworks, which is the idea that first was investigated in potential field and navigation function based methods \cite{khatib1986real}, \cite{rimon1992exact} and since then there has been a growing trend in the idea of integrating planning and control algorithms. In \cite{ghita2012trajectory} they propose a planning and control method for car-like robots in cell-decomposed environments, which although is a fully automatic algorithm, is not a complete one. In \cite{conner2003composition} they consider a polygonal partition of the environment and use vector fields in each polygon to guide the robot along the desired direction, and then in \cite{belta2005discrete} they designed a framework for automatically generating control laws in polygonal environments, which improved the main idea of \cite{conner2003composition} from the computational and compositional view. In \cite{danielson2016path} they design a set of local controllers for moving a robot with a linear model, while computing the required positive invariant sets for satisfying the input and output constraints on the dynamical system. In \cite{tedrake2009lqr} they design a planning algorithm that uses linear quadratic regulator controllers and feedback policies for stabilizing the planned trajectories at the goal configuration.

One of the challenging questions about providing control laws for robots is how to obtain a control, when both the safety and stability properties are important and may have conflict with each other. This question has been investigated recently in some works, such as \cite{intro5}, \cite{intro6} and \cite{intro7}, where the problem of having conflict between safety and stability purposes is solved by mediating them through a quadratic program (QP).


Our contributions in this work would be: 

This paper is structured as follows: In section ~\ref{section:} some necessary definitions are presented. Then the problem formulation for both first and second order systems, and our proposed method for solving them are given in sections III and IV. Simulation results for each of the systems are shown in section V, and then finally in section VI the concluding remarks and the future works of this research are stated.




%%%% control barrier and Lyapunov functions
% Control Barrier Function based quadratic programs with application to bipedal robotic walking
* Barrier functions, first utilized in numerical optimization methods [7], [23], are continuous functions whose values approach infinity when the state approaches the boundary of a set. Lyapunov-like barrier functions have been established; that is, employing derivatives of barrier functions guarantees the invariance of set.

% Control barrier function based quadratic programs with application to adaptive cruise control
* Barrier functions - first utilized in optimization [7] - are now common throughout the control and verification literature due to their natural relationship with Lyapunov functions [23], [27], their ability to provably establish invariance of sets [6], [19], [20], [28], and their relationship to multi-objective control [18]. Control Lyapunov Functions (CLFs), as pioneered in [21], [5], [22] and studied in depth in [8], utilize Lyapunov functions together with inequality constraints on their derivative to establish entire classes of controllers that stabilize a given system. 

% Path planning using positive invariant sets
* Positive invariant set definition: A set is positive invariant if any closed-loop state trajectory that starts inside the set remains in the set for all future times.


%%%% Our proposed method
% Discrete abstractions for robot motion planning and control in polygonal environments
We focus on polygonal (planar) environments and start by constructing a triangulation of the environment. The triangulation provides a partition of the environment in a manner that complex environments can be thought of as compositions of simple triangles. This geometric decomposition reduces the complexity of motion generation as it allows focusing on the complexity of the robot dynamics defined in triangles










-------------------------------------------------------------

%%%% Comparison with previous works?
% LQR-Trees: Feedback Motion Planning on Sparse Randomized Trees
% Present a feedback motion planning algorithm that combines locally valid linear quadratic regulator (LQR) controllers into a nonlinear feedback policy which probabilistically covers the reachable area of a bounded state space with a region of stability, certifying that all initial conditions that are capable of reaching the goal will stabilize to the goal. we present the LQR-Tree algorithm, which uses locally optimal linear feedback control policies to stabilize planned trajectories computed by local trajectory optimizers, and computational Lyapunov verification based on a sum-of-squares method to create the funnels.
% Possible disadvantage: nonlinear formulation

% Triangulation-based path planning for a mobile robot
% Present a triangulation-based path planning algorithm for a mobile robot. A circular robot operating in a planar polygonal environment cluttered with polygonal obstacles is considered. Constructs a triangulation graph, representing the topological connectivity of the free space, from which safe paths from the start to the goal can be found.



% Trajectory planning for a car-like robot by environment abstraction
% This work proposes a fully automatic planning and control strategy for solving a navigation problem for a car-like robot with non-negligible size and constraint control inputs. The approach uses cell decompositions for abstracting the robot behavior to a final state description on which the planning problem is solved. The originality of our method mainly comes from the iterative procedure for finding a feasible path based on cell decompositions. Although the approach is not complete, it benefits from a fully-automatic planning and control strategy and from a reduced computational complexity.
% An interesting control policy for nonholonomic systems is designed in [12,30], where the environment is abstracted into a finite set of curved surface cells, and the continuity in command angle is ensured by increasing the space dimension of the model. Besides complexity issues, a drawback of the proposed method is the lack of an automated strategy for abstracting the environment. The planning part of our approach is based on cell decomposition methods, and it ensures an output trajectory that can be followed by the car-like robot. The trajectory following part consists of an adapted version of the virtual vehicle approach proposed in [31,32].

% Path planning using positive invariant sets
% Present an algorithm for steering the output of a linear system from a feasible initial condition to a desired target, while satisfying input constraints and non-convex output constraints. The system input is generated by a collection of local linear state-feedback controllers. The path planning algorithm selects the appropriate local controller using a graph search, where the nodes of the graph are the local controllers and the edges of the graph indicate when it is possible to transition from one local controller to another without violating input or output constraints. We present two methods for computing the local controllers. The first uses a fixed-gain controller and scales its positive invariant set to satisfy the input and output constraints. We provide a linear program for determining the scale-factor and a condition for when the linear program has a closed-form solution. The second method designs the local controllers using a semi-definite program that maximizes the volume of the positive invariant set that satisfies state and input constraints.
% Possible disadvantages: no guarantee on existence of path, no stability

% Composition of Local Potential Functions for Global Robot Control and Navigation
% Presents a method of composing simple control policies, applicable over a limited region in a dynamical system's free space, such that the resulting composition completely solves the navigation and control problem for the given system operating in a constrained environment. The goal is to develop feedback control strategies that allow for automatic deployment of control policies in constrained environments, such that the resulting control system instantiates a natural, provably correct behavior for systems operating near their dynamic capabilities. The approach we propose is based on decomposing the free space into cells, and solving the navigation and control problem for specific cells, basing control only on local information. The overall control policy is formed by composing the local control policies in a way that guarantees the overall performance. We take inspiration from the work of [8], and the use of sequential composition to control a juggling robot. In their application, complex behaviors over a large domain were obtained by composing control policies designed to function over limited domains. Their work required hand-tuning and development of the specific control policy domains, and required the user to specify the deployment scheme. This paper also builds on prior work of the second author using sequential composition as a programming tool to specify robot motion programs for planar robots [9], [10].

% Discrete abstractions for robot motion planning and control in polygonal environments
% present a computational framework for automatic generation of provably correct control laws for planar robots in polygonal environments. Using polygon triangulation and discrete abstractions, we map continuous motion planning and control problems specified in terms of triangles to computationally inexpensive finite state transition systems. In this framework, powerful discrete planning algorithms in complex environments can be seamlessly linked to automatic generation of feedback control laws for robots with under-actuation constraints and control bounds.
% Among all literature on robot planning and control, this work is closest related to [7], [8]. In these papers, the authors consider a polygonal partition of a planar configuration space and assign vector fields in each polygon so that initial states in each polygon can only flow to a neighbor through the corresponding common facet. Even though the motivating ideas are the same, in this paper we use fundamentally different tools, which are much more suited for computation and composition than the one presented in [7], [8].



----------------------------------------------------------------------------------------------------------------------------------------------------------------------
%%%% Composition of Local Potential Functions for Global Robot Control and Navigation
% Conventional robot architectures have separated the planning and control problem to a degree that provably correct planning algorithms offer no guarantees of dynamical performance. 
% The desired path to follow may not be possible to perfectly track, due to the constraints in the form of kinematic and dynamical limitations on achievable states. 
% An early method to integrate planning and control was based on potential fields [4]. Unfortunately, most potential field constructions suffer from the well documented local minima problem [5], [6]. Koditschek [6] developed a local minima free potential field method for control by mapping a class of obstacles to a model space and generating a minimum free potential function over the model space; this potential function was termed a navigation function. 


%%%% Trajectory planning for a car-like robot by environment abstraction
% Path planning and controlling of mobile robots draws increasing attention during the last two decades [1–3]. 
% The classical navigation problem consists of finding a control strategy in order to move a mobile robot from a start position to a desired one, without colliding with static obstacles. In the majority of such problems, an optimal solution is rather unlikely to be found, or the approach would be too expensive from the computational point of view.
% Navigation problems for mobile robots are usually solved in two steps, namely a path planning part, whose output is a reference trajectory for the robot, and a trajectory following part, whose output is a continuous controller that keeps the robot as close as possible to the reference trajectory.
% Path planning methods can be divided into two main categories, based on the employed mathematical model of the environment. Thus, some approaches directly work on the initial (continuous) environment, while others abstract the environment to a finite (discrete) representation. In the first case, the solutions are usually based on potential and navigation functions [17,18], where the planning and the control part are interconnected. The main difficulty consists in designing such functions without local minima and in handling non-spherical obstacles. In the second case, the approaches can be further divided into ones that use roadmaps (e.g., visibility graphs or Voronoi diagrams) [2,3], and others based on decomposition of the free space into cells (geometric shapes) [2,3,19,20]. 
% It is worth mentioning that for holonomic robots an optimal solution from the point of view of the length of the resulted path can be obtained based on visibility graphs [2,3]. A drawback of visibility-graph-based methods is the closeness of robot’s trajectory to obstacles. For some nonholonomic robots, an optimal solution can be found in a free infinite environment, e.g. such approaches for car-like robots are described in [21–24].
% The task of designing control laws that allow tracking given reference trajectories reduces to a control problem with constraints issued by the robot dynamics. However, it is possible that for nontrivial dynamics the trajectory tracking cannot be enforced. Therefore, for handling specific robots, path planning and controller design are interconnected, either by restricting the path planning based on the control capabilities of the robot, or by iterating both parts until a feasible solution is obtained.



%%%% Discrete abstractions for robot motion planning and control in polygonal environments
% Motion planning for robots in geometrically complex environments is a fundamental problem that received a lot of attention lately [24], [25], [6]. 
% The vast literature on this topic can be divided in two schools of thought. 
% The first focuses on the complexity of the environment, while assuming that the robot is fully actuated with no control bounds, or ”free flying” [24]. This is the main simplifying assumption in most of the path planning methods based on navigation techniques. 
% Continuous paths from initial to final configurations in the robot task space can be found using roadmap methods such as Voronoi diagrams, visibility graphs, and freeway methods [24], potential fields [19], [21], [24], [37], or navigation functions [20], [36]. Discrete paths can also be built using cellular decompositions of the configuration space [24] or probabilistic roadmaps [18], [26]. Even though these methods produce paths that are perfectly valid from a planning perspective, the robot might fail to accomplish the task because of under-actuation and control constraints. The other school of thought focuses on the detailed dynamics or kinematics of the robot, while assuming trivial environments. Most of these methods are continuous and based on nonlinear control theory. To properly deal with nonholonomic systems, some of these approaches are differential geometric [23], [43] or exploit concepts such as flatness [39]. Other approaches use different types of input parametrization leading to multi-rate [42] or time varying [29], [9], [34], [28] control laws. Finally, discontinuous control laws obtained by combining different controllers [22] or by applying nonsmooth transformations of the state space [10], [3] have been proposed. While properly dealing with issues such as under-actuation and nonholonomy, such approaches face serious algorithmic challenges in complex environments [41]. 




%%%% Sampling-Based Temporal Logic Path Planning
% Motion planning is a fundamental problem that has received a lot of attention from the robotics community [1]. 
% The goal is to generate a feasible path for a robot to move from an initial to a final configuration while avoiding obstacles.
% Exact solutions to this problem are intractable, and relaxations using potential fields, navigation functions, and cell decompositions are commonly used [2]. These approaches, however, become prohibitively expensive in high dimensional configuration spaces. Sampling-based methods were proposed to overcome this limitation.




%%%% Path planning using positive invariant sets
% Recently, there has been much work on sampling-based motion planning, where the search space of possible trajectories is reduced to a graph search amongst randomly selected samples [2], [3], [4]. There are still many practical challenges in applying these methods to systems with complex dynamics in high dimensional spaces, since the algorithms must account for the dynamics and constraints of the system. 


















==> preamble/compactLists.tex <==
% set compact lists
\setlist[1]{\labelindent=\parindent}
\setlist[1]{topsep=3pt, itemsep=0pt}


==> preamble/courseFormatting.tex <==
%make underscore work without escaping in text mode
\usepackage{underscore}

%Common style that will be used for titles
\newcommand{\titlestyle}{\color{DodgerBlue3}\sffamily}

%Perfect 1-inch margins
\usepackage[margin=1in]{geometry}
\usepackage[medium,compact]{titlesec}
\usepackage{longtable}
\titleformat*{\section}{\titlestyle \Large}
\titleformat*{\subsection}{\titlestyle \large \itshape}

%Lists (requires enumitem package):
%Font for description
\setlist[description]{font=\color{DodgerBlue3}}
%Compact lists
\setlist[1]{\labelindent=\parindent}
\setlist[1]{topsep=3pt, itemsep=0pt}

%Format main title
\let\prevtitle\title
\renewcommand{\title}[1]{\prevtitle{\titlestyle #1}}
\let\prevauthor\author
\renewcommand{\author}[1]{\prevauthor{\titlestyle #1}}
\let\prevdate\date
\renewcommand{\date}[1]{\prevdate{\titlestyle #1}}

%Displayed quotations (used to define an environment for function specification)
\usepackage{csquotes}


%Include code
\usepackage{listings}

%formatting for the description of a function's input/output arguments
\mdfdefinestyle{functionspecification}{%
linecolor=DodgerBlue3,
rightline=false, topline=false, bottomline=false,
outerlinewidth=1.35,
roundcorner=10pt,
innerleftmargin=1.2em,
innertopmargin=0.3em,
innerbottommargin=0.3em,
leftmargin=1pt,
skipabove=0.5em,  
skipbelow=0.5em,  
backgroundcolor=white}

\newcommand{\dstar}{$\bigstar$}


==> preamble/courseProblemSet.tex <==
\input{preamble/courseFormatting}

%Facilities for markers file
% open file the beginning of the document
\AtBeginDocument{%
  \newwrite\markerstream
  \immediate\openout\markerstream=\jobname.mlg
}
% close the file at the end of the document
\AtEndDocument{%
  \immediate\closeout\markerstream
}
%definition similar to \typeout, but for markers
\makeatletter
\newcommand{\markerout}[1]{\begingroup \set@display@protect \immediate \write \markerstream {#1}\endgroup}
\makeatother

\usetikzlibrary{intersections}

\titleformat{\section}{\titlestyle\large\bfseries}{Problem \thesection:}{0.5ex}{}
%\titleformat{\subsection}{\normalfont\bfseries}{Problem \thesubsection:}{0.5ex}{}
\titleformat{\paragraph}[runin]{\titlestyle\normalsize\bfseries}{}{2pt}{}

%Macro for paragraph header for preparation steps to questions
%\newcommand{\preparation}{\smallskip\par\noindent\textbf{\titlestyle Preparation.~}}

\newcommand{\preparation}[1][]{%
\smallskip\par\noindent%
\textbf{\titlestyle Preparation \displayifnotempty{~(}{#1}{)}.~}}

%New custom counter for question
\newcounter{question}[section]

%Macro for writing points for the current question to the log file.
\newcommand{\pointmarker}{\typeout{Question points marker [\thesection.\thequestion] [\questionpoints]}}

\makeatletter
%Makes questions that:
%- are automatically numbered using the format <sectionNumber>.<questionNumber>
%- can be referred to using the usual \label-\ref mechanism
%- if the optional argument is not empty, this is displayed in parenthesis (typically, this will be a \points{n} or a \optional command). If the optional argument is empty, a single point is silently added to the point counter.
\newcommand{\question}[1][]{%
\smallskip\par\noindent%
\refstepcounter{question}\zerovar{\questionpoints}%
\sbox\boxifnotempty{\textbf{\titlestyle #1}}% for some reason, if the box is saved inside the \textbf{\titlestyle ...} (to avoid repeating the style), the box counts as empty for \ifempty, so I need to repeat the style here.
\textbf{\titlestyle Question \thesection.\thequestion\displayifnotempty{~(}{\usebox{\boxifnotempty}}{)}.~}%
\ifempty{\usebox{\boxifnotempty}}{\increasepoints{1}}%
\def\@currentlabel{{\thesection.\thequestion}}\pointmarker}
\makeatother
\newcommand{\hintquestion}[1]{\paragraph{Hint
    for question \ref{#1}:~}}
\newcommand{\hint}{\paragraph{Hint:~}}

\newcommand{\answer}[1][]{\smallskip\leavevmode\\\noindent\textbf{Answer \thesection.\thequestion#1:~}}

\newcommand{\updated}[1]{{\color{red} #1}}

\newcolorlabel{labeloptional}{DodgerBlue3}
\newcommand{\optional}{\labeloptional{optional}}
\newcolorlabel{labelprovided}{Orange1}
\newcommand{\provided}{\labelprovided{provided}}
\newcolorlabel{labelvideo}{OliveDrab3}
\newcommand{\video}{\labelvideo{video}}
\newcolorlabel{labelimage}{DarkOrchid2}
\newcommand{\image}{\labelimage{image}}
\newcolorlabel{labelcode}{SlateBlue2}
\newcommand{\code}{\labelcode{code}}
\newcolorlabel{labelscan}{Chocolate3}
\newcommand{\scan}{\labelcode{scan}}
\newcolorlabel{labelnew}{OliveDrab3}
\newcommand{\lbnew}{\labelnew{new}}

%\newcommand{\optional}{{\titlestyle optional}}

\tikzset{point/.style={inner sep=0pt,fill=black,circle,minimum size=4pt}}

%macros for keeping track of points (total, and for current question)
\zerovar{\totalpoints}
\zerovar{\bonuspoints}
\zerovar{\questionpoints}
\newcommand{\increasepoints}[1]{\addtovar{\totalpoints}{#1}\addtovar{\questionpoints}{#1}}
\newcommand{\points}[1]{#1 point\ifthenelse{\equal{#1}{1}}{}{s}\increasepoints{#1}}
\makeatletter
\newcommand{\totalpointswithbonus}[1]{\pgfmathparse{\storeddef{totalpoints}+#1}\pgfmathresult\typeout{Total points marker [\pgfmathresult]}}
\makeatother

\newstoreddef{totalpoints} %remember total number of points in aux file

% answer boxes
\newcommand{\vspaceboxdelta}{3mm}
\newcommand{\vspacebox}[1]{\par\bigskip{\tikz{\useasboundingbox (0,-\vspaceboxdelta) rectangle (\textwidth,#1\baselineskip); \draw[gray!20!white,line width=3pt] (-\vspaceboxdelta,-\vspaceboxdelta) rectangle (\textwidth+2*\vspaceboxdelta,#1\baselineskip+\vspaceboxdelta);}}\par}
\newcommand{\vspaceoneline}{\vspacebox{2}}
\newcommand{\vspacetwolines}{\vspacebox{3}}
\newcommand{\vspacethreelines}{\vspacebox{4}}
\newcommand{\vspacefourlines}{\vspacebox{5}}

% text fields
\newcommand{\textrowfield}[1]{\par\noindent#1: \enspace\hrulefill}

% formatting for the description of a function's input/output arguments
\usepackage[framemethod=tikz]{mdframed}
\mdfdefinestyle{functionspecification}{%
linecolor=DodgerBlue3,
rightline=false, topline=false, bottomline=false,
outerlinewidth=1.35,
roundcorner=10pt,
innerleftmargin=1.2em,
innertopmargin=0.3em,
innerbottommargin=0.3em,
leftmargin=1pt,
skipabove=0.5em,  
skipbelow=0.5em,  
backgroundcolor=white}
\mdfdefinestyle{classspecification}{%
linecolor=DarkOliveGreen3,
rightline=false, topline=false, bottomline=false,
outerlinewidth=1.35,
roundcorner=10pt,
innerleftmargin=1.2em,
innertopmargin=0.3em,
innerbottommargin=0.3em,
leftmargin=1pt,
skipabove=0.5em,  
skipbelow=0.5em,  
backgroundcolor=white}
%Note: I was not able to avoid duplication of options.

\newenvironment{functionspecification}{\markerout{Marker function [start]}\begin{mdframed}[style=functionspecification]}
{\markerout{Marker function [end]}\end{mdframed}}%
\newenvironment{classspecification}{\markerout{Marker class [start]}\begin{mdframed}[style=classspecification]}
{\markerout{Marker class [end]}\end{mdframed}}%
%\NewEnviron{fdescription}{\par\noindent{\titlestyle Description}: \BODY\markerout{Marker text [description] [start]^^J\BODY^^JMarker text [description] [end]}\par}
\NewEnviron{fdescription}{\par\noindent{\titlestyle Description}: \BODY\markerout{Marker text [description] [start]^^J\BODY^^JMarker text [description] [end]}\par}
\newenvironment{cdescription}{\fdescription}{\endfdescription}
\NewEnviron{frequirements}{\par\noindent{\titlestyle Requirements}: \BODY\markerout{Marker text [requirements] [start]^^J\BODY^^JMarker text [requirements] [end]}\par}
\newcommand{\cname}[1]{\noindent{\titlestyle Class name}: \var{#1}\par}
\newenvironment{finputs}{\markerout{Marker argument_group [start] [inputs]}\noindent{\titlestyle Input arguments}\begin{itemize}}{\end{itemize}\markerout{Marker argument_group [end]}}
\newenvironment{foutputs}[1][Output]{\markerout{Marker argument_group [start] [outputs]}\noindent{\titlestyle #1 arguments}\begin{itemize}}{\end{itemize}\markerout{Marker argument_group [end]}}
\newcommand{\freturns}[2][]{\noindent{\titlestyle Returns}: \var{#2}\displayifnotempty{ (type }{\var{#1}}{)}}
\newcommand{\argument}[4][]{\markerout{Marker argument [start]}\markerout{Marker argument [name] [#2]}\var{#2} %
  \ifnotempty{#1#3}{(\ifnotempty{#3}{\markerout{Marker argument [dimensions] [#3] [#4]}dim. \vardim{#3}{#4}\ifnotempty{#1}{, }}%
  \displayifnotempty{\markerout{Marker argument [type] [#1]}type }{\var{#1}}{})}\markerout{Marker argument [end]}}
\newcommand{\argumentscalar}[2][]{\argument[#1]{#2}{}{}}
\newcommand{\fheader}[3][]{\noindent{\titlestyle Header}: \function[#1]{#2}{#3}\par}
\newcommand{\fname}[2][Function]{\noindent{\titlestyle #1 name}: \var{#2}\par}
\newcommand{\ffilename}[1]{\noindent{\titlestyle File name}: \file{#1}\par}
\newcommand{\functionheader}[3][]{\markerout{Marker function_header [#1] [#2] [#3]}\function[#1]{#2}{#3}\par}

%ROS node specification
\newenvironment{nodespecification}{\begin{mdframed}[style=functionspecification]%
\newcommand{\filename}[1]{\par{\titlestyle File name:} \file{##1}}
\renewenvironment{description}{\par\noindent{\titlestyle Description:}}{\par}%
\newenvironment{subscribers}{\par\noindent{\titlestyle Subscribes to topics:}}{}%
\newenvironment{publishers}{\par\noindent{\titlestyle Publishes to topics:}}{}%
%
}{\end{mdframed}}

\newcommand{\rostopic}[2]{\var{#1} (type \var{#2})}

% Macros for questions where student need to draw on axes
\newcommand{\drawingaxes}[1][]{\draw[gray] (-5,-5) grid (5,5);
  \draw[very thick, -latex] (-5.7,0) -- (5.7,0);
  \draw[very thick, -latex] (0,-5.7) -- (0,5.7); #1}
\newcommand{\shifteddrawingaxes}[1][]{
  \begin{scope}[xshift=15cm]
    \drawingaxes[#1]
  \end{scope}
}

\newcommand{\drawexercise}[2][]{\begin{center}
\begin{tikzpicture}[scale=0.6]
  \node[text width=5cm,anchor=west]{#2};
  \shifteddrawingaxes[#1]
\end{tikzpicture}
\end{center}
}


==> preamble/courseProblemSetSectionsLettered.tex <==
%Change format of numbering for questions to letters instead of numbering
\renewcommand{\thequestion}{\alph{question}}


==> preamble/courseSyllabus.tex <==
 \input{preamble/courseFormatting}


\newlength{\topicwidth}
\newlength{\topicdatewidth}
\setlength{\topicdatewidth}{19mm}
\newlength{\duewidth}
\setlength{\duewidth}{23mm}

%Create a topictable environment from the longtable environment
\newenvironment{topictable}[1][2cm]%
{\newcommand{\picswidth}{#1}\setlength{\topicwidth}{\textwidth-\picswidth-\topicdatewidth-\duewidth-12.5mm}%
\setcounter{topic}{1}\begin{longtable}{p{\picswidth}p{\topicwidth}p{\topicdatewidth}p{\duewidth}}}%
{\end{longtable}}

%Prepare counter and relative macros for handling array of class dates
\newcount\i
\pgfmathsetcount{\i}{0}
\def\classdate{\pgfprint{\classdatearray[\i]}\global\advance\i 1\relax}

%Counters for topic and subtopic
\newcounter{topic}
\newcounter{subtopic}

%Topichead
\def\topichead#1#2#3{\rowcolor{SlateGray1}{\setcounter{subtopic}{1}\rule{0pt}{16pt}\titlestyle Topic \arabic{topic}\addtocounter{topic}{1}} & \multicolumn{3}{l}{{\titlestyle #1:} #2 \rule[-8pt]{0pt}{12pt}}\\\tikz[overlay]{\node[anchor=north west,inner sep=0pt]{\includegraphics[width=\picswidth,keepaspectratio]{figures/#3}};}}
\def\firstsubtopic#1{ & \makecell[{{p{\topicwidth}}}]{\rule{0pt}{14pt}#1}\addtocounter{subtopic}{1}}
\def\subtopic#1{\\ \cmidrule{2-4} & \makecell[{{p{\topicwidth}}}]{#1}\addtocounter{subtopic}{1}}
%\def\topicdate#1{& \makecell[{{p{\topicdatewidth}}}]{#1}}
\newcommand{\topicdate}[1][\classdate]{& \makecell[{{p{\topicdatewidth}}}]{#1}}
\def\due#1{& \makecell[{{p{\duewidth}}}]{#1}}
\def\endtopic{\\}
\newcolorlabel{labelhw}{Orange1}
\newcommand{\hwdue}[1]{\labelhw{HW #1}}
\newcolorlabel{paperdue}{Tomato1}
\newcolorlabel{examdue}{Tomato1}
\newcolorlabel{labelMH}{DodgerBlue3}
\newcommand{\mhday}{\labelMH{M-H}~}
\newcolorlabel{labelqz}{Sienna3}
\newcommand{\qzdue}[1]{\labelqz{QZ #1}~}

%TODO: Add automatic test to check if a subtopic is the first subtopic, and adjust the formatting accordingly.
%The subtopic counter is already there, but due to conflicts with the tabular environment, I was not able to include the test inside the \subtopic macro.
%\def\tpctest{\noalign{\ifnum\value{subtopic}=1{}\else{\hrule}\fi}}


==> preamble/generateGraphLocalization <==
#!/usr/bin/env python
# Note: in the list of node and edge quantities: first element is the name to use in the command name,
# the second is the one to use in the definition

import os
f=open('graphLocalization.tex','w')

f.write('% This file was generated by the script'+os.path.basename(__file__)+'\n')
f.write('% Do not modify this file directly\n\n')

f.write('% Notation for nodes\n')
nodeIndexList=['i','j']
nodeStateDoubleList=[['R','R'],['T','T']]
for index in nodeIndexList:
    for state in nodeStateDoubleList:
        f.write('\\newcommand{\\'+state[0]+index+'}{'+state[1]+'_{'+index+'}}\n')
        f.write('\\newcommand{\\d'+state[0]+index+'}{\\dot{'+state[1]+'}_{'+index+'}}\n')
        f.write('\\newcommand{\\dd'+state[0]+index+'}{\\ddot{'+state[1]+'}_{'+index+'}}\n')
    f.write('\n')
f.write('\n')

edgeIndexList=['ij','ji']
edgeStateDoubleList=[['R','R'],['T','T'],['beta','\\beta'],['c','c'],['d','d'],['q','q'],['l','\\lambda'],['varphi','\\varphi'],['g','g']]

f.write('% Notation for edges\n')
for index in edgeIndexList:
    for state in edgeStateDoubleList:
        f.write('\\newcommand{\\'+state[0]+index+'}{'+state[1]+'_{'+index+'}}\n')
    f.write('\n')
f.write('\n')

f.write('% Notation for edges, measured quantities\n')
for index in edgeIndexList:
    for state in edgeStateDoubleList:
        f.write('\\newcommand{\\t'+state[0]+index+'}{\\tilde{'+state[1]+'}_{'+index+'}}\n')
        f.write('\\newcommand{\\dt'+state[0]+index+'}{\\dot{\\tilde{'+state[1]+'}}_{'+index+'}}\n')
    f.write('\n')
f.write('\n')

f.write('% Node state differences\n')
f.write('\\newcommand{\\xjmi}{x_j-x_i}\n')
f.write('\\newcommand{\\vjmi}{v_j-v_i}\n')
f.write('\\newcommand{\\nxjmi}{\\norm{\\xjmi}}\n')
f.write('\n')

f.write('% Notation for desired quantities\n')
quantityTripleList=[['x','x','i'],['x','x','j'],['beta','\\beta','ij'],['d','d','ij']]
for quantity in quantityTripleList:
    f.write('\\newcommand{\\'+quantity[0]+'g'+quantity[2]+'}{'+quantity[1]+'_{g,'+quantity[2]+'}}\n')

f.close()






        


==> preamble/generateNotation <==
#!/usr/bin/env python
import string
import os
f=open('notation.tex','w')

f.write('% This file was generated by the script'+os.path.basename(__file__)+'\n')
f.write('% Do not modify this file directly\n\n')

f.write('% Shortand notation for vectors and their derivatives\n')
for c in string.ascii_lowercase+string.ascii_uppercase:
    f.write('\\providecommand{\\v'+c+'}{\\vct{'+c+'}}\n')
    f.write('\\providecommand{\\dv'+c+'}{\\dot{\\vct{'+c+'}}}\n')
    f.write('\\providecommand{\\tv'+c+'}{\\tilde{\\vct{'+c+'}}}\n')
    f.write('\\providecommand{\\dtv'+c+'}{\\dot{\\tilde{\\vct{'+c+'}}}}\n')
f.write('\n')
for c in [['beta','\\beta'],['sigma','\\sigma']]:
    f.write('\\providecommand{\\v'+c[0]+'}{\\boldsymbol{'+c[1]+'}}\n')
    f.write('\\providecommand{\\dv'+c[0]+'}{\\dot{\\boldsymbol{'+c[1]+'}}}\n')
f.write('\n')
for c in ['e']:
    f.write('\\providecommand{\\t'+c+'}{\\tilde{'+c+'}}\n')
f.write('\n')

f.write('% Shortand notation for derivatives and bold of symbols\n')
for c in [['gamma','\\gamma'],['Delta','\Delta']]:
    f.write('\\providecommand{\\d'+c[0]+'}{\\dot{'+c[1]+'}}\n')
    f.write('\\providecommand{\\dd'+c[0]+'}{\\ddot{'+c[1]+'}}\n')
    f.write('\\providecommand{\\v'+c[0]+'}{\\bm{'+c[1]+'}}\n')
f.write('\n')


f.write('% Shortand notation for matrices\n')
for c in string.ascii_uppercase:
    f.write('\\providecommand{\\m'+c+'}{\\vct{'+c+'}}\n')
f.write('\n')

f.write('% Shortand notation for calligraphic upper case letters\n')
for c in string.ascii_uppercase:
    f.write('\\providecommand{\\c'+c+'}{\\mathcal{'+c+'}}\n')
f.write('\n')

f.write('% Shortand notation for some tilded symbols and their derivatives\n')
symbolDoubleList=[['x','x'],['y','y'],['varphi','\\varphi']]
for symbol in symbolDoubleList:
    f.write('\\providecommand{\\t'+symbol[0]+'}{\\tilde{'+symbol[1]+'}}\n')
    f.write('\\providecommand{\\dt'+symbol[0]+'}{\\dot{\\tilde{'+symbol[1]+'}}}\n')
f.write('\n')

f.close()


==> preamble/graphLocalization.tex <==
% This file was generated by the scriptgenerateGraphLocalization
% Do not modify this file directly

% Notation for nodes
\newcommand{\Ri}{R_{i}}
\newcommand{\dRi}{\dot{R}_{i}}
\newcommand{\ddRi}{\ddot{R}_{i}}
\newcommand{\Ti}{T_{i}}
\newcommand{\dTi}{\dot{T}_{i}}
\newcommand{\ddTi}{\ddot{T}_{i}}

\newcommand{\Rj}{R_{j}}
\newcommand{\dRj}{\dot{R}_{j}}
\newcommand{\ddRj}{\ddot{R}_{j}}
\newcommand{\Tj}{T_{j}}
\newcommand{\dTj}{\dot{T}_{j}}
\newcommand{\ddTj}{\ddot{T}_{j}}


% Notation for edges
\newcommand{\Rij}{R_{ij}}
\newcommand{\Tij}{T_{ij}}
\newcommand{\betaij}{\beta_{ij}}
\newcommand{\cij}{c_{ij}}
\newcommand{\dij}{d_{ij}}
\newcommand{\qij}{q_{ij}}
\newcommand{\lij}{\lambda_{ij}}
\newcommand{\varphiij}{\varphi_{ij}}
\newcommand{\gij}{g_{ij}}

\newcommand{\Rji}{R_{ji}}
\newcommand{\Tji}{T_{ji}}
\newcommand{\betaji}{\beta_{ji}}
\newcommand{\cji}{c_{ji}}
\newcommand{\dji}{d_{ji}}
\newcommand{\qji}{q_{ji}}
\newcommand{\lji}{\lambda_{ji}}
\newcommand{\varphiji}{\varphi_{ji}}
\newcommand{\gji}{g_{ji}}


% Notation for edges, measured quantities
\newcommand{\tRij}{\tilde{R}_{ij}}
\newcommand{\dtRij}{\dot{\tilde{R}}_{ij}}
\newcommand{\tTij}{\tilde{T}_{ij}}
\newcommand{\dtTij}{\dot{\tilde{T}}_{ij}}
\newcommand{\tbetaij}{\tilde{\beta}_{ij}}
\newcommand{\dtbetaij}{\dot{\tilde{\beta}}_{ij}}
\newcommand{\tcij}{\tilde{c}_{ij}}
\newcommand{\dtcij}{\dot{\tilde{c}}_{ij}}
\newcommand{\tdij}{\tilde{d}_{ij}}
\newcommand{\dtdij}{\dot{\tilde{d}}_{ij}}
\newcommand{\tqij}{\tilde{q}_{ij}}
\newcommand{\dtqij}{\dot{\tilde{q}}_{ij}}
\newcommand{\tlij}{\tilde{\lambda}_{ij}}
\newcommand{\dtlij}{\dot{\tilde{\lambda}}_{ij}}
\newcommand{\tvarphiij}{\tilde{\varphi}_{ij}}
\newcommand{\dtvarphiij}{\dot{\tilde{\varphi}}_{ij}}
\newcommand{\tgij}{\tilde{g}_{ij}}
\newcommand{\dtgij}{\dot{\tilde{g}}_{ij}}

\newcommand{\tRji}{\tilde{R}_{ji}}
\newcommand{\dtRji}{\dot{\tilde{R}}_{ji}}
\newcommand{\tTji}{\tilde{T}_{ji}}
\newcommand{\dtTji}{\dot{\tilde{T}}_{ji}}
\newcommand{\tbetaji}{\tilde{\beta}_{ji}}
\newcommand{\dtbetaji}{\dot{\tilde{\beta}}_{ji}}
\newcommand{\tcji}{\tilde{c}_{ji}}
\newcommand{\dtcji}{\dot{\tilde{c}}_{ji}}
\newcommand{\tdji}{\tilde{d}_{ji}}
\newcommand{\dtdji}{\dot{\tilde{d}}_{ji}}
\newcommand{\tqji}{\tilde{q}_{ji}}
\newcommand{\dtqji}{\dot{\tilde{q}}_{ji}}
\newcommand{\tlji}{\tilde{\lambda}_{ji}}
\newcommand{\dtlji}{\dot{\tilde{\lambda}}_{ji}}
\newcommand{\tvarphiji}{\tilde{\varphi}_{ji}}
\newcommand{\dtvarphiji}{\dot{\tilde{\varphi}}_{ji}}
\newcommand{\tgji}{\tilde{g}_{ji}}
\newcommand{\dtgji}{\dot{\tilde{g}}_{ji}}


% Node state differences
\newcommand{\xjmi}{x_j-x_i}
\newcommand{\vjmi}{v_j-v_i}
\newcommand{\nxjmi}{\norm{\xjmi}}

% Notation for desired quantities
\newcommand{\xgi}{x_{g,i}}
\newcommand{\xgj}{x_{g,j}}
\newcommand{\betagij}{\beta_{g,ij}}
\newcommand{\dgij}{d_{g,ij}}


==> preamble/graphicsExport.tex <==
% activate externalization of figures
\usetikzlibrary{external}

\tikzexternalize 

%command to insert a Beamer frame from a sketch and externalize with the same name 
\newcommand{\insertsketchframe}[1]{\section{$\mathrm{#1}$}%
\tikzsetnextfilename{#1}%
  \begin{tikzpicture}[scale=0.7]%
    \input{sketch/#1}%
  \end{tikzpicture}%
\endpgfgraphicnamed%
}

%command to insert a Beamer frame from a tikz drawing and externalize with the same name 
\newcommand{\inserttikzframe}[1]{\section{$\mathrm{#1}$}%
\tikzsetnextfilename{#1}%
\input{tikz/#1}%
\endpgfgraphicnamed%
}


==> preamble/math.tex <==
%AMS typesetting
\makeatletter
\@ifpackageloaded{amsmath}{}{%
\usepackage[cmex10]{amsmath}%
}
\makeatother
\usepackage{mathtools}
\usepackage{amssymb,amsfonts}
\makeatletter
\@ifundefined{proof}{%
\usepackage{amsthm}%
}{}
\makeatother

\usepackage{mathtools}

%Common math statements environments
\makeatletter
\@ifundefined{theorem}{
\newtheorem{theorem}{Theorem}
\newtheorem{corollary}{Corollary}
\newtheorem{proposition}{Proposition}
\newtheorem{lemma}{Lemma}
\newtheorem{remark}{Remark}
\newtheorem{fact}{Fact}
}{}
  %SIAM article classes give their own Definition and Remark environments
\@ifundefined{definition}{
  \newtheorem{definition}{Definition}
}
% \@ifundefined{remark}{
%   \newtheorem{remark}{Remark}
% }
\makeatother
\newtheorem{problem}{Problem}
\newtheorem{assumption}{Assumption}
\newtheorem{property}{Property}
\newcommand{\rmss}[1]{_{\textrm{#1}}}

%%% Local Variables: 
%%% mode: latex
%%% End: 


==> preamble/preambleHelp.tex <==
\section*{Markup and commenting commands}
Use the command \var{\textbackslash newcommenter\{cname\}\{color\}} to enable the following commands (substitute \var{cname} with your pseudonim of choice, e.g., \var{rtron}, and \var{color} with a color name supported by the \var{xcolor} package):
\begin{itemize}
\item \var{\textbackslash cname\{comment\}}: typeset a colored comment labeled with the pseudonim.
\item \var{\textbackslash atcname}: use this to refer to another commenter.
\item \var{\textbackslash cnamehl\{comment\}\{text\}}: use this to highligth a portion of the text and comment on it.
\end{itemize}
Examples after using \var{\textbackslash newcommenter\{rtron\}\{Green3\}}:
\begin{itemize}
\item \var{\textbackslash rtron\{Ignore this comment\}} produces \rtron{Ignore this comment}.
\item \var{\textbackslash atrtron} produces \atrtron.
\item \var{\textbackslash rtronhl\{Sentence is obvious\}\{The sky is blue\}} produces \rtronhl{Sentence is obvious}{The sky is blue}
\end{itemize}

Use the command \var{\textbackslash sout} to strike out text.

==> preamble/roboticsHelp.tex <==
This file introduces commands for drawing axes and cameras.

\begin{itemize}
\item \var{ax[label][opts]\{refid\}\{x\}\{y\}\{rot\}} Draws a pair of 2-D axes. \var{refid} can be the used to put labels and third axes.
\item \var{axup[label_rotation]\{refid\}\{label\}\{rot\}}
\item \var{axlabels\{refid\}\{label1\}\{label2\}}
\item \var{camera[label]\{refid\}\{x\}\{y\}\{rot\}}
\item \var{gpoint\{coordinates\}\{label\}\{rot\}}
\end{itemize}

